Numerical Matrix Decomposition

In 1954, Alston S. Householder published \textit{Principles of Numerical Analysis}, one of the first modern treatments on matrix decomposition that favored a (block) LU decomposition-the factorization of a matrix into the product of lower and upper triangular matrices. And now, matrix decomposition has become a core technology in machine learning, largely due to the development of the back propagation algorithm in fitting a neural network. The sole aim of this survey is to give a self-contained introduction to concepts and mathematical tools in numerical linear algebra and matrix analysis in order to seamlessly introduce matrix decomposition techniques and their applications in subsequent sections. However, we clearly realize our inability to cover all the useful and interesting results concerning matrix decomposition and given the paucity of scope to present this discussion, e.g., the separated analysis of the Euclidean space, Hermitian space, Hilbert space, and things in the complex domain. We refer the reader to literature in the field of linear algebra for a more detailed introduction to the related fields. Keywords: Existence and computing of matrix decompositions, Floating point operations (flops), Low-rank approximation, Pivot, LU/PLU decomposition, CR/CUR/Skeleton decomposition, Coordinate transformation, ULV/URV decomposition, Rank decomposition, Rank revealing decomposition, Update/downdate, Tensor decomposition.

==> chapter-coordinate.tex <==
\newpage 
\part{Special Topics}

\newpage
\chapter{Transformation in Matrix Decomposition}\label{section:coordinate-transformation}
\begingroup
\hypersetup{
	linkcolor=structurecolor,
	linktoc=page,  % page: only the page will be colored; section, all, none etc
}
\minitoc \newpage
\endgroup

\lettrine{\color{caligraphcolor}W}


\begin{problemset}

\end{problemset}




==> chapter-id-bid-iid.tex <==










\subsection{Quantitative Problem Example}\label{section:iid_quantaprob}
After developing the intervened interpolative decomposition algorithm, one may get confused about why it is so important and curious about the applications it can be applied in practice.
It is well known that large quantitative hedge funds and asset managers have been recruiting a large number of data miners and financial engineers in order to build effective alphas, and the number of alpha components might climb into the millions or perhaps billions \citep{tulchinsky2019finding}. 
%It is known that WorldQuant has been hiring plenty of data miners and financial engineers to create effective alphas and the number of alpha factors can grow into millions or even billions \citep{tulchinsky2019finding}. 
%In industry-level quantitative companies, e.g., WorldQuant, BlackRock, Risk Parity, and Guotai Junan Securities, the number of alpha factors can grow into millions or even billions. 
Therefore, using all the alphas or a large fraction of the alpha pool to create a meta-alpha can be problematic for the following reasons: 
%As a result, creating a meta-alpha from all of the alphas or a large fraction of the alpha pool might be troublesome for the following reasons: 
a). If we use the same alphas (all the time), some illiquid alphas with low volume can be traded heavily. This will make the strategy meaningless due to volume constraint; 
b). Using too many alphas can cause overfitting and the out-of-sample (OS) performance will be poor due to the overfitting;
c). Many alphas might be mutually dependent, and certain machine learning algorithms, e.g., neural networks, to find the meta-strategy from the whole bunch of alphas can find their limitations caused by the multi-linear problems;
d). Finding trading signals from the full alpha pool can be time-consuming because of the limited computing resources;
e). We always want to find a different subset of alphas to explore different strategies with low correlation so as to avoid market risks.
For the five reasons mentioned above, there is an urgent need to develop algorithms to select a small subset of alphas from the whole bunch of it so as to reduce overfitting, make the end strategy more scalable, and find the results within a certain amount of time.
It is trivial to select an appropriate subset by the \textit{RankIC} metric (see definition below), i.e., we select the alphas having the highest RankIC values. However, the problems still remain that the selected subset can not represent the whole pool of alphas, and the selected alphas may be mutually dependent.

Our goal is to find as many representative alpha factors with desirable performance as possible. The selected subset of alphas is representative in the sense that the small subset of alphas can be used to reconstruct other alphas with a small error.
The traditional ID algorithm, either using a \textit{Randomized algorithm} \citep{liberty2007randomized} or a Bayesian approach we have discussed above, can only help to find the representative ones. However, the end choices may seem to select alphas with low performance.
Using the IID method, on the other hand, can help find the representative (that can reconstruct other alphas with small error) and the desirable (high RankIC scores) alphas at the same time.

\subsubsection{Formulaic Alphas}
Previously, 101 formulaic short-term alpha factors were released by WorldQuant, a quantitative investment management company, in 2016 \citep{kakushadze2016101}. Since then, the 191 alpha factors from Guotai Junan Securities \citep{guotaijunan2017} have also been welcomed by many investors and institutions.
These formulaic alpha factors are derived  from various data variables of each stock, e.g., the volume, price, volatility, volume-weighted average price (vwap), and so on.
As the name implies, a formulaic alpha is a type of alpha that can be expressed as a formula or a mathematical expression. For example, a \textit{mean-reversion} alpha can be expressed in terms of a mathematical expression as follows:
$$
\text{Alpha =  }- \left( \text{close(today) $-$close(5$\_$days$\_$ago ) } \right)/ 
\text{close(5$\_$days$\_$ago)}.
$$
In this sense, we take the opposite action as indicated by the closing price: to short if the price  has risen during the previous five days, and we go long otherwise. At a high level, the alpha value indicates the trend of the price in the days to come; the higher the alpha value for each stock, the more likely it is that the stock's price will rise in the next few days.



\subsubsection{Evaluation Metrics}
Let $r_{t}$ denote the yield rate of stock $s$ on $t$-day. Suppose further 
$p_t$ is asset closing price at time $t$ where $t\in \{1,2,\ldots, T\}$, the
return of the asset at time $t$ can be obtained by the following
equation:
\begin{equation}
	r_t = \frac{p_t - p_{t-1}}{p_t}.
\end{equation}
We use the Rank information coefficient (\textit{RankIC}) to evaluate the effectiveness of an alpha:
\begin{equation}
	\text{RankIC}(\ba, \br^h)=\text{Spearman}(\ba, \br^h),
\end{equation}
where $\text{Spearman}(\cdot)$ indicates the Spearman correlation, $\ba$ is the sequence of an alpha, $\br^h$ is the sequence of the return value with holding period $h$ such that the $i$-th element of $\br^h$ represent the daily return of $h$ days later. The RankIC then can be used as an indicator of the importance of each alpha factor and plugged into Equation~\eqref{equation:posterior_IID} directly.



\subsection{Real-World Application}\label{section:iid_experiments}

For each stock $s$  (i.e., $s\in \{1,2,\ldots, S\}$ where $S$ is the total number of stocks), we have a matrix $\bA_s$ with shape $\bA_s\in \real^{N\times D}$ where $N$ is the number of alphas and $D$ is the number of dates so that each row of $\bA_s$ is regarded as an alpha series. We want to select a subset of the alphas (here we assume $M$ out of the $N$ alphas are selected). The RankIC between each alpha series and the delayed return series with horizon $h=1$ is then taken as the \textit{important value} directly, higher RankIC indicates higher priority.



\begin{table}[h]
\centering
\small 
\setlength{\tabcolsep}{5.8pt}
\begin{tabular}{llllll}
	\hline
	Ticker & Type & Sector & Company &  Avg. Amount \\ \hline
	SH601988   & Share & Bank               & Bank of China Limited    &  427,647,786  \\
	SH601601   & Share & Public Utility    & China Pacific Insurance (Group)   & 819,382,926 \\
	SH600028    & Share & Public Utility & China Petroleum \& Chemical Corporation              &  748,927,952\\
	SH600016    & Share & Bank    & China Minsheng Banking Corporation &285,852,414  \\
	SH601186    & Share & Public Utility    & China Railway Construction Corporation  & 594,970,588\\
	SH601328    & Share & Bank & Bank of Communications Corporation &  484,445,915  \\
	SH601628     & Share & Public Utility & China Life Insurance Company Limited&368,179,861  \\
	SH601939    & Share   & Bank      & China Construction Bank Corporation &527,876,669  \\
	\hline
	SH510300    & ETF   & CSI 300         & Huatai-PineBridge CSI 300 ETF  &1,960,687,059  \\
	SH510050      & ETF   & CSI 50 & ChinaAMC China CSI 50 ETF    &2,020,385,879  \\
	\hline
\end{tabular}
\vspace{-0.25cm} 
\caption{Summary of the underlying portfolios in the China market, 10 assets totally. The average amount (in the currency of RMB) is calculated in the period of the test set.}
\label{table:iid_cn_data_summary}		
\end{table}



\paragraph{Dataset}
To evaluate the algorithm and demonstrate the main advantages of the IID method, 
we conduct experiments with different analysis tasks; 10 assets from China market, and various industrial segments including Bank, Public Utility, and ETF.
We obtain publicly available data from tushare \footnote{\url{https://tushare.pro/}.}. 
We obtain data for a 3-year period, i.e., 2018-07-18 to 2021-07-05 (720 trading days), where the data between 2018-07-18 and 2020-07-09 is considered training set (480 calendar days); 
while data between 2020-07-10 and 2021-07-05 is taken as the test set (240 trading days).
The underlying portfolios are summarized in Table~\ref{table:iid_cn_data_summary} and Figure~\ref{fig:bid_iid_datasets_ashare} shows the series of different assets where
we initialize each portfolio with a unitary value for clarity.
The assets are chosen by selecting the ones with high amount (random 10 assets among the first highest 50 in China market during the period of test set) so that there is a small trading limitation.

We obtain 78 alphas from the 101 formulaic alphas \citep{kakushadze2016101}, 94 alphas from the 191 formulaic alphas \citep{guotaijunan2017}, and 19 self-made alphas. The alphas are selected to have a reasonable value, neither too large nor too small.
In this sense, the alpha matrix $\bA_s$ is of shape $214\times 480$ for each asset.  




In all scenarios, the same parameter initialization is adopted when conducting different tasks. 
Experimental evidence reveals that post processing procedure can increase performance to a minor level.
For clarification, we only provide the findings of the GBT and IID models after post processing.
In a wide range of experiments across various datasets, the IID model can select the important features (alphas) with higher priority while keeping the reconstructive error as small as possible
and leading to performance that is as good or better than the vanilla GBT method in low-rank ID approximation.

In order to measure
overall decomposition performance, we use mean squared error (MSE, Equation~\eqref{equation:idbid-per-example-loss}), which measures the similarity between the observed and reconstructive matrices; the smaller the better performance. 




\begin{figure*}[h]
\centering  
\vspace{-0.2cm} 
\subfigtopskip=2pt 
\subfigbottomskip=0pt 
\subfigcapskip=-2pt 
\subfigure[Convergence of the models on the 
SH510050, SH510300, SH601939, SH601628, and SH601328 datasets, measured by the data fit (MSE). The algorithm almost converges in less than 100 iterations.]{\includegraphics[width=1\textwidth]{imgs_bid/iid_alpha_convergence.pdf} \label{fig:iid_alpha_convergence}}
\subfigure[Averaged autocorrelation coefficients of samples of $y_{kl}$ computed using Gibbs sampling on the 
SH510050, SH510300, SH601939, SH601628, and SH601328 datasets.]{\includegraphics[width=1\textwidth]{imgs_bid/iid_alpha_autocorrelation.pdf} \label{fig:iid_alpha_autocorrelation}}
\vspace{-0.3cm} 
\caption{Convergence results (upper), and sampling mixing analysis (lower) on the SH510050, SH510300, SH601939, SH601628, and SH601328 datasets for a latent dimension of $K=10$.
}
\label{fig:allresults_bids_ard}
\end{figure*}
\paragraph{Hyperparameters}
In these experiments, we use  $a=-1, b=1,\alpha_\sigma=0.1, \beta_\sigma=1$, ($\{\mu_{kl}\}=0, \{\tau_{kl}\}=1$) for both GBT and IID models.
The adopted parameters are  uninformative and weak prior choices and the models are insensitive to them.
The observed or unobserved variables are initialized from random draws as long as these hyperparameters are fixed since this initialization method provides a better initial guess of the correct patterns in the matrices.
In all scenarios, we run the Gibbs sampling 1,000 iterations with a burn-in of 100 iterations and a thinning of 5 iterations as the convergence analysis shows the algorithm can converge in fewer than 100 iterations.

\begin{table}[]
\centering
\vspace{-0.35cm} 
\tiny
\setlength{\tabcolsep}{3.7pt}
\begin{tabular}{lllllllllll}
\hline 
& SH601988 & SH601601 & SH600028 & SH600016 & SH601186 & SH601328 & SH601628 & SH601939 & SH510300 & SH510050\\
\hline 
GBT Min & 5.235 & 5.814 & 5.235 & \textbf{6.381}& 5.819 & 5.700 & 5.734 & 5.785 & 5.462 & 6.297 \\
IID Min & \textbf{4.567} &\textbf{5.700}& \textbf{4.843} & 6.490 & \textbf{5.104} & \textbf{5.658} & \textbf{5.445} & \textbf{5.435} & \textbf{4.876} & \textbf{5.767} \\
GBT Mean & 6.476 & \textbf{7.367} & 6.764 & 8.053 & 7.066 & 7.250 & 7.206 & 7.242 & 6.769 & 7.776 \\
IID Mean & \textbf{6.239} & 7.449 & \textbf{6.664} & \textbf{7.831} & \textbf{6.558} & \textbf{7.081} & \textbf{7.002} & \textbf{7.031} & \textbf{6.450} & \textbf{7.492} \\
\hline
\end{tabular}
\vspace{-0.3cm} 
\caption{Minimal and mean MSE measures after burn-in across different iterations for GBT and IID models on the 10 alpha matrices from 10 assets. In all cases, $K=10$ is set as the latent dimension. 
In most cases, the results of IID converge to a smaller value than the GBT model.}
\label{table:comparis_gbt_iid_mse}
\vspace{-0.1cm} 
\end{table}




\begin{figure*}[h]
\centering  
\vspace{-0.3cm} 
\subfigtopskip=2pt 
\subfigbottomskip=9pt 
\subfigcapskip=-1pt 
\subfigure[10 Different portfolios where we initialize each portfolio with a unitary value for clarity.]{\includegraphics[width=0.45\textwidth]{imgs_bid/bid_iid_datasets_ashare.pdf} \label{fig:bid_iid_datasets_ashare}}
\subfigure[Portfolio values with the same strategy by using different alphas via comparative selection models.]{\includegraphics[width=0.45\textwidth]{imgs_bid/bid_iid_portfolio_ashare.pdf} \label{fig:bid_iid_portfolio_ashare}}
\vspace{-0.3cm} 
%	\includegraphics[width=0.75\textwidth]{imgs/bid_iid_portfolio_ashare.pdf}
\caption{Portfolio values of the 10 assets (left), and the portfolio values (right) of different methods where we split by in-sample and out-of-sample periods, and initialize with unitary value for each period. The IID performs better in the out-of-sample period (see also Table~\ref{table:iid_selected_mean_ic}).}
\label{fig:bid_iid_portfolio_ashare}
\end{figure*}


\subsubsection{Convergence and Comparative Analysis}
We first show the rate of convergence over iterations on different assets. Due to space limit, we omit the convergence results for the first 5 assets, and only present results for SH510050, SH510300, SH601939, SH601628, SH601328 portfolios. Results for the other assets are qualitatively similar.

We run GBT and IID models with latent dimension $k=10$ for the 5 datasets where $214$ is the full rank of the matrices, and the error is measured by MSE.
Figure~\ref{fig:iid_alpha_convergence} shows the rate of convergence over iterations. Figure~\ref{fig:iid_alpha_autocorrelation} shows autocorrelation coefficients of samples computed using Gibbs sampling. We observe that the mixings of the IID are close to those of GBT. The coefficients are less than 0.1 when the lags are greater than 10, indicating that the Gibbs sampler mixes well. 
In all experiments, the algorithm converges in less than 100 iterations.
We also observe that the IID model does not converge to a larger error than the vanilla GBT model, though we put more emphasis on selecting the columns with high RankIC. Table~\ref{table:comparis_gbt_iid_mse} presents the minimal MSE and mean MSE after burn-in across different iterations for GBT and IID models on the 10 alpha matrices from 10 assets. In most cases, the IID can even converge to a smaller MSE value.






\begin{algorithm}[!htb] 
\caption{Alpha selection for portfolio allocation. Gibbs sampler for GBT and GBTN ID models. 
Select holding period $h$, number of alphas to select $M$.
} 
\label{alg:iid_alpha_selection}  
\begin{algorithmic}[1] 
\State Split the alpha matrix for in-sample (IS) and out-of-sample (OS) evaluations: 
$$
\bA_{\text{in}} = \bA_s[:,0:D_{\text{in}}] \in \real^{N\times D_{\text{in}}}, \gap 
\bA_{\text{out}} = \bA_s[:,D_{\text{in}}+1:D]\in \real^{N\times (D-D_{\text{in}})};
$$
\State Using ID to decide the alphas to be selected  on matrix $\bA_{\text{in}}^\top$, with the selected indices $\bmm$:
$$
\widehat{\bA}_{\text{in}} = \bA_s[\bmm,0:D_{\text{in}}] \in \real^{\textcolor{mylightbluetext}{M}\times D_{\text{in}}}, \gap 
\widehat{\bA}_{\text{out}} = \bA_s[\bmm,D_{\text{in}}+1:D]\in \real^{\textcolor{mylightbluetext}{M}\times (D-D_{\text{in}})};
$$
\For{$m=1$ to $M$}
\State Using the $m$-th IS alpha vector $\ba_m=\widehat{\bA}_{\text{in}}[m,:]\in \real^{D_{\text{in}}}$ to decide the weight $\bw$ and interception $b$ via ordinary least squares (OLS) so that the MSE between the prediction $\ba_m^\top\bw_m +b_m$ and the shifted return vector $\br^h$ is minimized, i.e., minimizing $\text{MSE}(\ba_m^\top\bw_m +b_m, \br^h)$. The weight and interception are then used in OS evaluation.
\EndFor
\For{$d=1$ to $D-D_{\text{in}}$}
\State On each day in the OS period, we use the mean evaluation of each prediction from the $M$ alphas to decide to go long or not, i.e., to long if $\sum_{m=1}^M \ba_m^\top\bw_m +b_m >0$; and do nothing otherwise since we restrict the analysis to  long-only portfolios.
Though we employ a long-only portfolio, we can favor a \textit{market-neutral strategy}: we open long positions only when we anticipate that at least half of the stocks will rise on the following $h$ day, and we weight each stock equally.
%Though we apply long only portfolio, we can favor a somewhat \textit{market-neutral strategy}: we open long position only when we predict half of the stocks are rising on the following $h$ day; and we put equal weight on each stock.
\EndFor
\end{algorithmic} 
%\vspace{-0.1cm}
\end{algorithm}


\begin{table}[]
\centering
%\vspace{-0.4cm} 
\setlength{\tabcolsep}{7.5pt}
\small
\begin{tabular}{lllll}
\hline 
Methods & Highest RankIC & Randomized ID & BID with GBT & BID with IID \\
\hline
Mean RankIC & \textbf{0.1035}         & 0.0651        & 0.0553       & \textbf{0.0752}  \\
Mean Correlation & 0.2276$\downarrow$         & 0.5741$\downarrow$        & \textbf{0.1132}       & \textbf{0.1497}  \\
\hline
Sharpe Ratio (OS) & 1.0276 & 1.0544 & 0.5045 & \textbf{1.5721}  \\
Sharpe Ratio (IS) & \textbf{2.6511} & 1.3019 & 1.4965 & 2.3231  \\
\hline
Annual Return (OS) & 0.1043 & 0.0932 & 0.0484 & \textbf{0.1633}  \\
Annual Return (IS) & \textbf{0.4390} & 0.2281 & 0.2425 & 0.3805  \\
\hline
Max Drawdown (OS) & 0.0632 & \textbf{0.0373} & \textbf{0.0484} & \textbf{0.0552}  \\
Max Drawdown (IS) & \textbf{0.0892} & 0.1548 & 0.1232 & \textbf{0.0975}  \\
\hline
\end{tabular}
\vspace{-0.3cm} 
\caption{Mean RankIC and correlation of the selected alphas across various assets for different methods. A higher mean RankIC and a lower mean correlation are better. The IID method can find the trade-off between the mean RankIC and the mean correlation.
In all cases, \textit{IS} means in-sample measurements, and \textit{OS} means out-of-sample measurements. The symbol $\downarrow$ means the performance is extremely poor.  
}
\label{table:iid_selected_mean_ic}
\end{table}

\subsubsection{Quantitative Strategy}
After running the GBT and IID algorithms for computing the interpolative decomposition of the alpha matrix of each asset, we save the state vector $\br$ for each asset and select the 10 alphas that have largest mean selection during the 1,000 iterations (with a burn-in of 100 iterations, and thinning of 5 iterations). 
Then we follow the quantitative strategy in Algorithm~\ref{alg:iid_alpha_selection} (in which case $h=1$, $N=214$ alphas, $M=10$ alphas, $D=720$ trading days, and $D_{\text{in}}=480$ trading days).
The procedure shown in Algorithm~\ref{alg:iid_alpha_selection} is a very simple quantitative strategy. However, the algorithm can show precisely how the IID method can work in practice.


The strategy using the alphas selected by the  IID method is only slightly worse than the one selecting the \textit{highest RankIC} alphas for the in-sample (IS) performance in terms of Sharpe ratio, annual return, and maximum drawdown; however, the IID performs better in the out-of-sample (OS) scenario and this is what we actually want (see Table~\ref{table:iid_selected_mean_ic} and Figure~\ref{fig:bid_iid_portfolio_ashare}).
To evaluate the strategy, we also adopt the Randomized algorithm to compute the ID for comparison \citep{liberty2007randomized}, termed \textit{Randomized ID}. The Randomized ID performs even worse than BID with GBT (see Table~\ref{table:iid_selected_mean_ic}).
Though the IID does not select alphas with the highest RankIC values, this does not mean that the alpha selection procedure is meaningless for the following reasons:
1). \textit{Pool size}: We only use a small set of alpha pool that only contains 214 alpha factors. When the number of alphas is approaching millions or even billions, the alpha selection procedure is expected to work better. 
2). \textit{Correlation}: The mean correlation of selected alphas across the 10 assets of the  IID method is smaller than the highest RankIC method. In this sense, the alphas of the latter method have high correlation2 and a low diversity. If the correlated alphas have low a liquidity or perform poorly during a given period, the risk of the strategy can be enlarged.
3). \textit{Machine learning models}: In our test, we only use OLS to find the weight of each alpha. For more complex models, e.g., neural networks, the correlated alphas can cause multi-linear problems so that the performance and interpretability are hampered.
4). \textit{Diversification}: Even if selecting the alphas with the highest RankIC can work well in practice, we also want to diversify the strategies so that we are not exposed to specific risks.
The  IID method can help find different strategies.







==> chapter-theorylowrank.tex <==
\newpage
\chapter{Analysis of Low-Rank Approximation}
\begingroup
\hypersetup{
	linkcolor=structurecolor,
	linktoc=page,  % page: only the page will be colored; section, all, none etc
}
\minitoc \newpage
\endgroup


\begin{table}[]
\centering
%\scriptsize
%	\small 
\setlength{\tabcolsep}{8pt}
\begin{tabular}{l|lll}
\hline
Method & Reference & $1/p(n,k)$  & Time \\ \hline\hline
RRQR   & \citet{hong1992rank}        & $\sqrt{k(n-k)+\min\{k,n-k\}}$ &   $\mathcalO(n^k)$   \\ \hline
&           &           &      \\ \hline
\end{tabular}
\end{table}

\section{Preliminaries}

To understand this section, you have to read the Cholesky decomposition, QR decomposition, spectral decomposition, SVD firstly.

\begin{theoremHigh}[Gu and Eisenstat]
Given a matrix $\bA\in\real^{m\times n}$, let $l=\min\{m,n\}$ and $k\in\{1,2,\ldots,l\}$. Then there exists a reduced QR decomposition 
$$
\bA\bP = \bQ\bR,
$$ 
where $\bP$ is an $n\times n$ permutation matrix, $\bQ$ is an $m\times l$ matrix with orthonormal columns, and $\bR$ is an $l\times n$ upper triangular matrix with the following forms
$$
\bQ=
\begin{blockarray}{ccc}
& k     &  l-k \\
\begin{block}{c[cc]}
k&\bQ_{11} & \bQ_{12} \\
m-k&\bQ_{21} & \bQ_{22}\\
\end{block}%
\end{blockarray}%
,
\gap
\bR=
\begin{blockarray}{ccc}
& k     &  n-k \\
\begin{block}{c[cc]}
k&\bR_{11} & \bR_{12} \\
l-k&\bzero & \bR_{22}\\
\end{block}%
\end{blockarray},
$$
where 
\begin{align}
\sigma_k(\bR_{11})
&\geq 
\sigma_k(\bA) 
\frac{1}{\sqrt{1+k(n-k)}}, \label{equation:guen11}\\
\sigma_1(\bR_{22})
&\leq 
\sigma_{k+1}(\bA) \sqrt{1+k(n-k)},\label{equation:guen12} \\
\norm{\bR_{11}^{-1}\bR_{12}}_F 
&\leq \sqrt{k(n-k)}. \label{equation:guen13}
\end{align}
While, the reduced QR decomposition satisfy the above inequality, we do not know the cost of constructing such a factorization numerically. 
Further, we have the following inequality in which case the decomposition can be computed in $\mathcalO(mn^2)$ operations:
\begin{align}
\sigma_k(\bR_{11})
&\geq 
\sigma_k(\bA) 
\frac{1}{\sqrt{1+nk(n-k)}}, \label{equation:guen21}\\
\sigma_1(\bR_{22})
&\leq 
\sigma_{k+1}(\bA) \sqrt{1+nk(n-k)},\label{equation:guen22} \\
\norm{\bR_{11}^{-1}\bR_{12}}_F
&\leq \sqrt{n k(n-k)}. \label{equation:guen23}
\end{align}
\end{theoremHigh}
Equation~\eqref{equation:guen12} implies that $\bA$ can be well approximated by a low-rank matrix:
$$
\norm{
\bA - \begin{bmatrix}
\bQ_{11} \\
\bQ_{21} 
\end{bmatrix}
\begin{bmatrix}
	\bR_{11} & \bR_{12}
\end{bmatrix}
\bP^\top
}_2
\leq \epsilon \sqrt{1+k(n-k)}.
$$
And Equation~\eqref{equation:guen13} implies that the first $k$ columns of $\bA\bP$ form a well-conditioned basis for the entire column space of $\bA$ (within an accuracy of $\epsilon$).


\section{Rank-Revealing QR Decomposition}
We defined the numerical rank and exact rank in Definition~\ref{definition:effective-rank-in-svd} (p.~\pageref{definition:effective-rank-in-svd}). For simplicity, we do not give the full rank of the rank when it is clear from the context which one we are referring to.
\begin{lemma}[Rank-Revealing QR (RRQR)]\label{lemma:numerica_qr}
Given the reduced QR decomposition $\bA\bP=\bQ\bR$ of a matrix $\bA\in\real^{m\times n}$ with $m\geq n$ and $\bQ\in\real^{m\times n}$: 
$$
\bR=
\begin{blockarray}{ccc}
	& r     &  n-r \\
	\begin{block}{c[cc]}
		r&\bR_{11} & \bR_{12} \\
		n-r&\bzero & \bR_{22}\\
	\end{block}%
\end{blockarray}.
$$
If 
\begin{equation}\label{equation:rrqr_condition}
\sigma_{\min}(\bR_{11})\gg \sigma_{\max}(\bR_{22}) = O(\mu),
\end{equation}
where $\mu$ is the machine precision, then $\bA$ has numerical rank $r$.
In this case, the QR decomposition is called a \textit{rank-revealing QR (RRQR)} decomposition of $\bA$ for rank $r$.
\end{lemma}

\begin{proof}[of Lemma~\ref{lemma:numerica_qr}]
From Remark~\ref{remark:qr_inter_svd} (p.~\pageref{remark:qr_inter_svd}), we have 
$$
\sigma_{\min}(\bR_{11})\leq \sigma_r(\bA) \gap 
\text{and}
\gap
\sigma_{\max}(\bR_{22}) \geq \sigma_{r+1}(\bA),
$$
where $\sigma_i(\bA)$ is the $i$-th largest singular value of $\bA$. Therefore, it follows that 
$$
\sigma_r(\bA) \geq \sigma_{\min}(\bR_{11})
\geq \sigma_{\max}(\bR_{22})
\geq
\sigma_{r+1}(\bA)
=
O(\mu).
$$
This completes the proof by the definition of numerical rank (Definition~\ref{definition:effective-rank-in-svd}, p.~\pageref{definition:effective-rank-in-svd}).
\end{proof}
The above lemma tells us if we can find a column-pivoted QR decomposition with Equation~\eqref{equation:rrqr_condition}, then we find the rank-revealing QR decomposition.
Or, once the permutation matrix $\bP$ is found such that the Equation~\eqref{equation:rrqr_condition} satisfies, the numerical rank of $\bA$ is revealed.
The lemma also tells us that a gap between $\sigma_{\min}(\bR_{11})$
and $\sigma_{\max}(\bR_{22})$ implies a gap between $\sigma_r(\bA)$ and $\sigma_{r+1}(\bA)$.


We have shown in Section~\ref{section:nonunique-qr} (p.~\pageref{section:nonunique-qr}) that the reduced QR decomposition is unique up to the signs of rows of $\bR$. When $\bA$ does not have full rank, the (reduced) QR decomposition is not unique. However, we prove that $\sigma_{\min}(\bR_{11})$ and $\sigma_{\max}(\bR_{22})$ are unique. Then if we can find the  permutation $\bP$ such that Equation~\eqref{equation:rrqr_condition} satisfies, we can always find the RRQR up to numerical sense.
\begin{lemma}[Uniqueness of RRQR  up to Numerical Sense]\label{lemma:unique_rrqr_numsen}
Given a matrix $\bA\in\real^{m\times n}$ with $m\geq n$, a permutation matrix $\bP\in\real^{n\times n}$ and given rank $r$,  if $\sigma_{\min}(\bR_{11})\neq 0$, then the values of  $\sigma_{\min}(\bR_{11})$ and $\sigma_{\max}(\bR_{22})$ are uniquely determined by the QR decomposition of $\bA\bP$ even though the QR decomposition may not be unique.
\end{lemma}
\begin{proof}[of Lemma~\ref{lemma:unique_rrqr_numsen}]
Suppose two reduced QR decompositions of $\bA\bP$ are 
$$
\bA\bP =\bQ
\begin{bmatrix}
\bR_{11} & \bR_{12} \\
\bzero & \bR_{22}\\
\end{bmatrix}
=
\overline{\bQ}
\begin{bmatrix}
	\overline{\bR}_{11} & \overline{\bR}_{12} \\
	\bzero & \overline{\bR}_{22}\\
\end{bmatrix}.
$$
Then we have 
$$
\bP^\top\bA^\top\bA\bP=
\begin{bmatrix}
\bR_{11}^\top\bR_{11} & \bR_{11}^\top\bR_{12} \\
\bR_{12}^\top\bR_{11} & \bR_{12}^\top\bR_{12}+\bR_{22}^\top\bR_{22}
\end{bmatrix}
=
\begin{bmatrix}
\overline{\bR}_{11}^\top\overline{\bR}_{11} & \overline{\bR}_{11}^\top\overline{\bR}_{12} \\
\overline{\bR}_{12}^\top\overline{\bR}_{11} & \overline{\bR}_{12}^\top\overline{\bR}_{12}+\overline{\bR}_{22}^\top\overline{\bR}_{22}
\end{bmatrix}.
$$
Since $\sigma_{\min}(\bR_{11})^2 = \lambda_{\min} (\bR_{11}^\top\bR_{11})$ and 
$\sigma_{\min}(\overline{\bR}_{11})^2 = \lambda_{\min} (\overline{\bR}_{11}^\top\overline{\bR}_{11})$, 
we have $\sigma_{\min}(\bR_{11})=\sigma_{\min}(\overline{\bR}_{11})$.

On the other hand, since $\bR_{11}, \overline{\bR}_{11}$ have full rank, by Cholesky decomposition, $\bR_{11}^\top\bR_{11}$ and $\overline{\bR}_{11}^\top\overline{\bR}_{11}$ are positive definite.
From the fact that $\bR_{11}^\top\bR_{11}=\overline{\bR}_{11}^\top\overline{\bR}_{11}$
$\bR_{11}^\top\bR_{12}=\overline{\bR}_{11}^\top\overline{\bR}_{12}$, it can be shown that 
$\bR_{12}^\top\bR_{12}=\overline{\bR}_{12}^\top\overline{\bR}_{12}$. 
Therefore, 
we have $\bR_{22}^\top\bR_{22} = \overline{\bR}_{22}^\top\overline{\bR}_{22}$. This implies 
$
\sigma_{\max}(\bR_{22})
=
\sigma_{\max}(\overline{\bR}_{22}).
\footnote{In fact, we also have $\sigma_i(\bR_{11})$ and $\sigma_j(\bR_{22})$ for all $i,j$.}
$
This proves the lemma.
\end{proof}


\begin{theoremHigh}[Hong and Pan \citep{hong1992rank}]\label{theorem:qr_hongpan}
Given a matrix $\bA\in\real^{m\times n}$ with $m\geq n$ and $k\in\{1,2,\ldots,n\}$. Then there exists a reduced QR decomposition 
$$
\underset{m\times n}{\bA}\gaps\underset{n\times n}{\bP} = 
\underset{m\times n}{\bQ}\gaps \underset{n\times n}{\bR},
$$
where $\bP$ is an $n\times n$ permutation matrix, $\bQ$ is an $m\times n$ matrix with orthonormal columns, and $\bR$ is an $n\times n$ upper triangular matrix with the following forms
$$
\bQ=
\begin{blockarray}{ccc}
& k     &  n-k \\
\begin{block}{c[cc]}
k&\bQ_{11} & \bQ_{12} \\
m-k&\bQ_{21} & \bQ_{22}\\
\end{block}%
\end{blockarray}%
,
\gap
\bR=
\begin{blockarray}{ccc}
& k     &  n-k \\
\begin{block}{c[cc]}
k&\bR_{11} & \bR_{12} \\
n-k&\bzero & \bR_{22}\\
\end{block}%
\end{blockarray},
$$
where 
\begin{align}
\sigma_{\min}(\bR_{11})
&\geq 
\sigma_{\min}(\bP_1^\top\bV_1)\sigma_k(\bA) , \label{equation:hongpan11}\\
\sigma_{\max}(\bR_{22})
&\leq 
 \frac{1}{\sigma_{\min}(\bP_2^\top\bV_2)}\sigma_{k+1}(\bA),\label{equation:hongpan12} 
%\norm{\bR_{11}^{-1}\bR_{12}}_F 
%&\leq \sqrt{k(n-k)}, \label{equation:hongpan13}
\end{align}
and  $\bA$ admits the SVD $\bA=\bU\bSigma\bV^\top$, $\bP = [\bP_1, \bP_2]\in\real^{n\times n}$ and $\bV=[\bV_1,\bV_2]\in\real^{n\times n}$ such that $\bP_1, \bV_1\in\real^{n\times k}$. 
Moreover, we have 
\begin{equation}\label{equation:hongpan14}
\sigma_{\min}(\underbrace{\bP_1^\top\bV_1}_{\real^{k\times k}}) = \sigma_{\min}(\underbrace{\bP_2^\top\bV_2}_{\real^{(n-k)\times (n-k)}}).
\end{equation}
\end{theoremHigh}
\begin{proof}[of Theorem~\ref{theorem:qr_hongpan}]
Let $\widetildebU=[\widetildebU_1, \widetildebU_2] =\bU\bSigma$ where $\widetildebU_1\in\real^{m\times k}$ 
such that $\bA\bV = \widetildebU$ and $\bA = \widetildebU_1\bV_1^\top +\widetildebU_2\bV_2^\top$. Then we have 
$$
\sigma_{\min}(\bA\bP_1) = \sigma_{\min} (\widetildebU_1\bV_1^\top\bP_1 +\widetildebU_2\bV_2^\top\bP_1)
\stackrel{*}{\geq }
\sigma_{\min} (\widetildebU_1\bV_1^\top\bP_1)
\stackrel{\dagger}{\geq }
\sigma_{\min} (\widetildebU_1)
\sigma_{\min} (\bP_1^\top\bV_1)
$$
where the inequality ($\dagger$) follows from Theorem~\ref{theorem:weyl_ineq2_sings} (p.~\pageref{theorem:weyl_ineq2_sings}), and the inequality ($*$) follows from the Weyl theorem (Theorem~\ref{theorem:weyl}, p.~\pageref{theorem:weyl}) by letting $\bX=\widetildebU_1\bV_1^\top\bP_1$ and $\bY=\widetildebU_2\bV_2^\top\bP_1$ such that ($\bX^\top\bT=\bzero$)
$$
\begin{aligned}
\sigma_{\min}^2\left(\bX+\bY\right)
&=\lambda_{\min}\left((\bX+\bY)^\top(\bX+\bY)\right)\\
&=\lambda_{\min}\left(\bX^\top\bX+\bY^\top\bY\right)
\geq \lambda_{\min}\left(\bX^\top\bX\right)=
\sigma_{\min}^2\left(\bX\right).
\end{aligned}
$$

On the other hand, we also have 
$\sigma_{\min}(\bA\bP_1) = \sigma_{\min}\left(\bQ\begin{bmatrix}
	\bR_{11}\\\bzero 
\end{bmatrix}\right)
=
\sigma_{\min}(\bR_{11})
$
and 
$\sigma_{\min}(\widetildebU_1)=\sigma_k(\bA)$ where $\sigma_k(\bA)$ is the $k$-th largest singular value of $\bA$.
Combine above claims, we prove Equation~\eqref{equation:hongpan11}.

Further, since 
$
\widetildebU_2  =\bA\bV_2 = \bA\bP\bP^\top\bV_2 = \bQ\bR\bP^\top\bV_2
$,
we have 
$$
\sigma_{k+1}(\bA) =
\norm{\widetildebU_2}_2
=
\norm{\bR\bP^\top\bV_2}_2
\geq
\underbrace{\norm{\bR_{22}\bP_2^\top\bV_2}_2}_{\sigma_{\max}(\bR_{22}\bP_2^\top\bV_2)}
\geq 
\sigma_{\max}(\bR_{22}) \sigma_{\min} (\bP_2^\top\bV_2),
$$
where the last inequality is again from Theorem~\ref{theorem:weyl_ineq2_sings} (p.~\pageref{theorem:weyl_ineq2_sings}). This proves Equation~\eqref{equation:hongpan12}.

Finally, Equation~\eqref{equation:hongpan14} can be proved  via CS decomposition since $\bP^\top\bV$ is orthogonal. 
\end{proof}

\begin{remark}
Following the settings in Theorem~\ref{theorem:qr_hongpan}, by Remark~\ref{remark:qr_inter_svd} (p.~\pageref{remark:qr_inter_svd}), we have 
$$
\sigma_{\min}(\bR_{11})\leq \sigma_k(\bA) \gap 
\text{and}
\gap
\sigma_{\max}(\bR_{22}) \geq \sigma_{k+1}(\bA).
$$
Therefore, Equation~\eqref{equation:hongpan11} and \eqref{equation:hongpan12} can be further bounded as 
\begin{align}
\sigma_k(\bA)  
\geq 
\sigma_{\min}(\bR_{11})
&\geq 
\sigma_{\min}(\bP_1^\top\bV_1)\sigma_k(\bA) ,\\
\sigma_{k+1}(\bA)
\leq  
\sigma_{\max}(\bR_{22})
&\leq 
\frac{1}{\sigma_{\min}(\bP_2^\top\bV_2)}\sigma_{k+1}(\bA).
\end{align}
\end{remark}

\textcolor{red}{TODO: definition of $\sO_{n,k}$}

$\sL(\bA) $, the $n\times n$ submatrices of $\bA\in\real^{m\times n}$ with $m\geq n$.

$\bA(i^\prime)$, a principal submatrix of a square matrix $\bA$ with the $i$-th row and $i$-th column of $\bA$ deleted.

$(\bA)_{ij}$, $(\bA)_{i,:}$, $(\bA)_{:,j}$

Let $p=C(n,k)$,
$$
\bsigma(\bW) = 
\left( \sigma_{\min}(\bW_1), \sigma_{\min}(\bW_2), \ldots, \sigma_{\min}(\bW_p)\right)
$$

$$
p(n,k) = \mathop{\inf}_{\bW\in\sO_{n,k}} 
\left( \norm{\bsigma(\bW)}_{\infty}  \right).
$$
From the CS decomposition, we have 
$$
p(n,k) = p(n,n-k).
$$

We notice that when $k=1$, $p=C(n,1)=n$. Then 
$$
p(n,1)=
\mathop{\inf}_{\normtwo{\bv}=1} (\norminf{\bv}),
$$
where $\bv\in\real^n$ with $\normtwo{\bv}=1$.
\begin{lemma}[Value of $p(n,1)$]\label{lemma:bound_n1}
Given a vector $\bv\in\real^n$ with $\normtwo{\bv}=1$. Then we have 
$$
p(n,n-1) = p(n,1) = 
\mathop{\inf}_{\normtwo{\bv}=1} (\norminf{\bv}) = \frac{1}{\sqrt{n}}.
$$
\end{lemma}
\begin{proof}[of Lemma~\ref{lemma:bound_n1}]
It's trivial that $\norminf{\bv}\geq \frac{1}{\sqrt{n}}$ for every $\bv\in\real^n$ with $\normtwo{\bv}=1$. When $\bv=[\frac{1}{\sqrt{n}}, \frac{1}{\sqrt{n}}, \ldots, \frac{1}{\sqrt{n}}]$, then $\normtwo{\bv}=1$ and $\norminf{\bv}=\frac{1}{\sqrt{n}}$ that achieves the lower bound.
\end{proof}


Combine Theorem~\ref{theorem:qr_hongpan} and Lemma~\ref{lemma:bound_n1}, the following result follows immediately.
\begin{corollaryHigh}[Rank-One Deficient, $k=n-1$, \citep{golub1976rank}]\label{theorem:qr_hongpan_k1}
When $k=n-1$ in Theorem~\ref{theorem:qr_hongpan}, there exists a permutation $\bP$ so we have the  reduced QR decomposition 
$$
\underset{m\times n}{\bA}\gaps\underset{n\times n}{\bP} = 
\underset{m\times n}{\bQ}\gaps \underset{n\times n}{\bR}
$$
such that 
%$$
%\bQ=
%\begin{blockarray}{ccc}
%& n-1     & 1 \\
%\begin{block}{c[cc]}
%n-1&\bQ_{11} & \bq_{12} \\
%m-n+1&\bQ_{21} & \bq_{22}\\
%\end{block}%
%\end{blockarray}%
%,
%\gap
%\bR=
%\begin{blockarray}{ccc}
%& n-1     &  1 \\
%\begin{block}{c[cc]}
%n-1&\bR_{11} & \br_{12} \\
%1&\bzero & r_{nn}\\
%\end{block}%
%\end{blockarray},
%$$
%where 
\begin{align}
\sigma_{\min}(\bR_{11})
%&\geq 
%\sigma_{\min}(\bP_1^\top\bV_1)\sigma_{n-1}(\bA) 
\geq \frac{1}{\sqrt{n}}\sigma_{n-1}(\bA) 
, \\
\abs{r_{nn}}
%&\leq 
% \frac{1}{\bp_n^\top\bv_n}\sigma_{n}(\bA)
 \leq 
\sqrt{n}\sigma_{n}(\bA) ,
\end{align}
where $\bR_{11}\in\real^{(n-1)\times (n-1)}$.
%and  $\bA$ admits the SVD $\bA=\bU\bSigma\bV^\top$, $\bP = [\bP_1, \bp_n]\in\real^{n\times n}$ and $\bV=[\bV_1,\bv_n]\in\real^{n\times n}$ such that $\bP_1, \bV_1\in\real^{n\times (n-1)}$. 
%Moreover, we have 
%\begin{equation}\label{equation:hongpank1_4}
%\sigma_{\min}(\underbrace{\bP_1^\top\bV_1}_{\real^{(n-1)\times (n-1)}}) = \bp_n^\top\bv_n.
%\end{equation}
Further, if $\bv_n$ is the right singular vector associated with $\sigma_n(\bA)$, the permutation $\bP$ is given by $\abs{(\bP^\top\bv_n)_n} = \norminf{\bv_n}$, i.e., $\abs{\bp_n^\top\bv_n} = \norminf{\bv_n}$. This can be easily checked that $\abs{\bp_n^\top\bv_n} = \norminf{\bv_n} \geq \frac{1}{\sqrt{n}}$ since $\normtwo{\bv_n}=1$.
Moreover, if $\bA$ is numerically rank-one deficient, the QR decomposition of $\bA\bP$ is guaranteed to be an RRQR of $\bA$.
\end{corollaryHigh}
\textcolor{red}{TODO: the result is the backbone of \citet{chan1987rank}}


\begin{lemma}[Bound of $p(n,2)$]\label{lemma:bound_n2}
Given a semi-orthogonal matrix $\bV\in\sO_{n,2}$. Then we have 
$$
p(n,n-2) = p(n,2) = 
\mathop{\inf}_{\bV\in\sO_{n,2}} (\norminf{\bsigma(\bV)}) 
\geq
\sqrt{\left( 2-\sqrt{2} \sqrt{(n-2)/(n-1)}\right)\big/n}.
$$
\end{lemma}

\textcolor{red}{TODO}

\begin{corollaryHigh}[Rank-Two Deficient, $k=n-2$, \citep{golub1976rank}]\label{theorem:qr_hongpan_k2}
When $k=n-2$ in Theorem~\ref{theorem:qr_hongpan}, there exists a permutation $\bP$ so we have the  reduced QR decomposition 
$$
\underset{m\times n}{\bA}\gaps\underset{n\times n}{\bP} = 
\underset{m\times n}{\bQ}\gaps \underset{n\times n}{\bR}
$$
such that 
\begin{align}
\sigma_{\min}(\bR_{11})
\geq 
\sqrt{\left( 2-\sqrt{2} \sqrt{(n-2)/(n-1)}\right)\big/n} \cdot
\sigma_{n-2}(\bA) ,
\\
\sigma_{\max}(\bR_{22})
\leq 
\frac{1}{\sqrt{\left( 2-\sqrt{2} \sqrt{(n-2)/(n-1)}\right)\big/n}}  \cdot
\sigma_{n-1}(\bA),
\end{align}
where $\bR_{11}\in\real^{(n-2)\times (n-2)}$.
Further, if $\bV_2=[\bv_{n-1}, \bv_n]\in\real^{n\times 2}$ contains the two right singular vectors associated with $\sigma_{n-1}(\bA)$ and $\sigma_n(\bA)$, respectively, then the permutation matrix $\bP$ is given by $\sigma_{\min} (\bP^\top\bV_2)_{n-1:n, n-1:n}=\norminf{\bsigma(\bV_2)}$.
Moreover, if $\bA$ is numerically rank-two deficient, the QR decomposition of $\bA\bP$ is guaranteed to be an RRQR of $\bA$.
\end{corollaryHigh}


\begin{lemma}\label{lemma:det_ineq_mainqrrr}
Given a semi-orthogonal matrix $\bV\in\sO_{n,k}$ with $k<n$ and a permutation $\bP=\begin{bmatrix}
\bP_1\\
\bP_2 
\end{bmatrix}\in\real^{n\times n}$ with $\bP_2\in\real^{k\times n}$ such that
$$
\abs{\det(\bP_2\bV)}
=
\mathop{\max}_{\bV^\prime\in \sL(\bV)} \abs{\det(\bV^\prime)}.
$$
Then the following inequality holds:
$$
\mathop{\max}_{1\leq i\leq k}
\frac{\det (\bG(i^\prime))}{\det(\bG)} \leq n-r+1,
$$
where $\bG = (\bP_2\bV)(\bP_2\bV)^\top$.
\end{lemma}
\begin{proof}[of Lemma~\ref{lemma:det_ineq_mainqrrr}]
	content...
\end{proof}



\begin{theoremHigh}[General Deficiency, General $k$, \citep{hong1992rank}]\label{theorem:qr_hongpan_generalk}
When considering general $k$ in Theorem~\ref{theorem:qr_hongpan}
and using Lemma~\ref{lemma:det_ineq_mainqrrr},
there exists a permutation $\bP$  so we have the  reduced QR decomposition 
$$
\underset{m\times n}{\bA}\gaps\underset{n\times n}{\bP} = 
\underset{m\times n}{\bQ}\gaps \underset{n\times n}{\bR}
$$
such that 
\begin{align}
\sigma_{\min}(\bR_{11})
&\geq 
\frac{1}{ \sqrt{k(n-k) +\min\{k, n-k\}}} \cdot
\sigma_k(\bA) , \\
\sigma_{\max}(\bR_{22})
&\leq 
 \sqrt{k(n-k) +\min\{k, n-k\}} \cdot
 \sigma_{k+1}(\bA),
\end{align}
where $\bR_{11}\in\real^{k\times k}$, $\bA$ admits the SVD $\bA=\bU\bSigma\bV^\top$, $\bP = [\bP_1, \bP_2]\in\real^{n\times n}$ and $\bV=[\bV_1,\bV_2]\in\real^{n\times n}$ such that $\bP_1, \bV_1\in\real^{n\times k}$. 
Further, the permutation matrix $\bP$ is obtained by selecting an $(n-k)\times (n-k)$ submatrix of $\bV_2$ having the largest determinant in absolute value among all such submatrices of $\bV_2$, and permuting it to the  bottom of the matrix $\bP^\top\bV_2$.

Moreover, if $\bA$ has numerical rank $k$, then the QR decomposition of $\bA\bP$ is guaranteed to be an RRQR decomposition of  $\bA$.
\end{theoremHigh}

\begin{proof}[of Theorem~\ref{theorem:qr_hongpan_generalk}]
Write out the decomposition, we have 
$$
\bP^\top\bV = 
\begin{bmatrix}
\bP_1^\top \\
\bP_2^\top 
\end{bmatrix}
\begin{bmatrix}
\bV_1 &\bV_2 
\end{bmatrix}
=
\begin{bmatrix}
\bP_1^\top\bV_1 & \bP_1^\top\bV_2 \\ 
\bP_2^\top\bV_1 & \bP_2^\top\bV_2 
\end{bmatrix}
:=
\begin{blockarray}{ccc}
& k     &  n-k \\
\begin{block}{c[cc]}
k&\bZ_{11} & \bZ_{12} \\
n-k&\bZ_{21} & \bZ_{22}\\
\end{block}%
\end{blockarray},
$$
where $\sigma_{\min}(\bZ_{11})=\sigma_{\min}(\bZ_{22}):=\rho$ by the CS decomposition.
Following Theorem~\ref{theorem:qr_hongpan}, we wish to find a lower bound of $\rho$ when we choose $\bP$ such that 
\begin{equation}\label{equation:general_k_permchoo}
\abs{\det(\bP_2^\top\bV_2)}
=
\mathop{\max}_{\bV_2^\prime\in \sL(\bV_2)} \abs{\det(\bV_2^\prime)}.
\end{equation}
By \textcolor{red}{adjoint matrix formulas}, we have 
$$
\left(\frac{1}{\sigma_{\min}(\bZ_{22})}\right)^2=
\normtwo{\bZ_{22}^{-1}}^2 \leq \normF{\bZ_{22}^{-1}}^2
= 
\sum_{i=1}^{n-k} \left( \bZ_{22}^{-\top}\bZ_{22}^{-1} \right)_{ii}
=
\sum_{i=1}^{n-k}  \frac{\det(\bG(i^\prime))}{\det(\bG)},
$$
where $\bG=\bZ_{22}\bZ_{22}^\top$.
By Lemma~\ref{lemma:det_ineq_mainqrrr}  and Equation~\eqref{equation:general_k_permchoo}, we have
$$
\sum_{i=1}^{n-k}  \frac{\det(\bG(i^\prime))}{\det(\bG)}
\leq 
(n-k) \frac{\mathop{\max}_{1\leq i\leq n-k} \det (\bG(i^\prime))}{\det(\bG)}
\leq 
(n-k)(k+1).
$$
Therefore, we get the inequality
$$
\rho \geq  \frac{1}{\sqrt{(n-k)(k+1)}}
=\frac{1}{\sqrt{(n-k)k + (n-k)}}
.
$$
Apply this process on $\bZ_{11}=\bP_1^\top\bV_1$, we find the permutation such that 
$
\abs{\det(\bP_1^\top\bV_1)}
=
\mathop{\max}_{\bV_1^\prime\in \sL(\bV_2)} \abs{\det(\bV_1^\prime)}.
$ And we obtain 
$$
\rho \geq  \frac{1}{\sqrt{k(n-k+1)}}
=\frac{1}{\sqrt{(n-k)k + k}}
.
$$
We conclude the results.
\end{proof}

The above theorem tells us that the RRQR decomposition of $\bA$ can be obtained by selecting a $k\times k$ submatrix of $\bV_1$ having the largest determinant in absolute value among all such submatrices of $\bV_1$, and by permuting it to the top of the matrix $\bP^\top\bV_1$ (where $\bV_1\in\real^{n\times k}$ contains the first right singular vectors of $\bA$).

The theorem also tells us the lower bound for the polynomial function $p(n,k)$:
$$
p(n,k)=p(n,n-k)
\geq 
\frac{1}{ \sqrt{k(n-k) +\min\{k, n-k\}}}.
$$
When $k=1$, we get the result in Lemma~\ref{lemma:bound_n1} (p.~\pageref{lemma:bound_n1}).
However, when $k=2$, we find the lower bound in Lemma~\ref{lemma:bound_n2} (p.~\pageref{lemma:bound_n2}) is tighter. A comparison between the two functions,  $\sqrt{\left( 2-\sqrt{2} \sqrt{(n-2)/(n-1)}\right)\big/n}$ and $\left(1/{2(n-2)+2}\right)$, for different values of $n$ is shown in Figure~\ref{fig:rrqr_lower_k2}.

\begin{SCfigure}%[h]
\centering
\includegraphics[width=0.58\textwidth]{./imgs/rrqr_lower_k2.pdf}
\caption{Comparison of $\sqrt{\left( 2-\sqrt{2} \sqrt{(n-2)/(n-1)}\right)\big/n}$ and $\left(1/{2(n-2)+2}\right)$, when $k=2$ for different values of $n$. The former one provides a tighter bound.}
\label{fig:rrqr_lower_k2}
\end{SCfigure}

The RRQR decomposition of $\bA$ can be defined using other matrix norms. 
\begin{theoremHigh}[General Deficiency, General $k$, w.r.t., Frobeniu Norm, \citep{hong1992rank}]\label{theorem:qr_hongpan_generalk_frobenius}
When considering general $k$ in Theorem~\ref{theorem:qr_hongpan}
and using Lemma~\ref{lemma:det_ineq_mainqrrr},
there exists a permutation $\bP$  so we have the  reduced QR decomposition 
$$
\underset{m\times n}{\bA}\gaps\underset{n\times n}{\bP} = 
\underset{m\times n}{\bQ}\gaps \underset{n\times n}{\bR}
$$
such that 
\begin{align}
\normF{\bR_{11}^{-1}}  
&\leq 
\sqrt{k(n-k+1)} \big/
\sigma_k(\bA) , \\
\normF{\bR_{22}}
&\leq 
\sqrt{(n-k)(k+1)} \cdot
\sigma_{k+1}(\bA),
\end{align}
where $\bR_{11}\in\real^{k\times k}$.
\end{theoremHigh}

\textcolor{red}{TODO, prove}





\subsection{Type-I Greedy Algorithms}
\textcolor{red}{TODO: discussion of Type-I and Type-II}.

$$
(\text{P1}) \gap \mathop{\max}_{\bP} \sigma_{\min}(\bR_{11})
$$


\begin{algorithm}[h] 
\caption{Greedy-I} 
\label{alg:greedy-I} 
\begin{algorithmic}[1] 
\Require Matrix $\bA$ with size $m\times n $ and $m\geq n$; 
\State $\bA$ admits reduced QR $\bA=\bQ\bR$;
\State Input the low rank number $k$;
\State Set initial upper triangular matrix $\bR^{(0)}=\bR\in\real^{n\times n}$;
\For{$l=0$ to $k$}
\State 
\algoalign{
Denote $\bR^{(l)}$ as 
$$
\bR^{(l)} :=
\begin{blockarray}{ccc}
& l     &  n-l \\
\begin{block}{c[cc]}
l&\bX & \bY \\
n-l&\bzero & \bZ\\
\end{block}%
\end{blockarray},
$$
where $\bY = [\by_1, \by_2, \ldots, \by_{n-l}]$ and $\bZ = [\bz_1, \bz_2, \ldots, \bz_{n-l}]$ are the column partitions of $\bY$ and $\bZ$ respectively.
}
\State   ($A$). Find the next column $l+j$ from $\bR^{(l)}$ such that 
$$
\sigma_{\min} 
\left(\begin{bmatrix}
	\bX & \by _j \\
	\bzero & \bz_j
\end{bmatrix}
\right)
=
\mathop{\max}_{1\leq i\leq n-l} \sigma_{\min} 
\left(\begin{bmatrix}
\bX & \by _i \\
\bzero & \bz_i
\end{bmatrix}
\right).
$$
\State \algoalign{($B$). Exchange columns $(l+1)$ and $(l+j)$ of $\bR^{(l)}$, and re-triangularize it from the left with orthogonal transformations to get $\bR^{(l+1)}$.}
\EndFor
%\State Output $\bQ=[\bq_1, \ldots, \bq_n]$ and $\bR$ with entry $(i,k)$ being $r_{ik}$;


\end{algorithmic} 
\end{algorithm}

In iteration 0 of Greedy-I algorithm, we simply find the column with the largest norm.

\begin{lemma}\label{lemma:mini_sigma_appendcol}
Given a matrix $\bA\in\real^{n\times n}$ and  two vectors $\bb\in\real^{n}$, $\bc\in\real^k$ with $z=\normtwo{\bc}$. Then it follows that 
$$
\sigma_{\min} 
\left(
\begin{bmatrix}
\bA & \bb \\
\bzero & \bc 
\end{bmatrix}
\right)
=
\sigma_{\min} 
\left(
\begin{bmatrix}
	\bA & \bb \\
	\bzero & z 
\end{bmatrix}
\right),
$$
where $\sigma_{\min}(\bX)$ is the smallest singular value of $\bX$.
\end{lemma}
\begin{proof}[of Lemma~\ref{lemma:mini_sigma_appendcol}]
	Let 
$$
\bM_1 = 
\begin{bmatrix}
\bA & \bb \\
\bzero & \bc 
\end{bmatrix}
\gap
\text{and}
\gap 
\bM_2 = 
\begin{bmatrix}
	\bA & \bb \\
	\bzero & z 
\end{bmatrix}.
$$
Since the eigenvalues of $\bX^\top\bX$ are equal to the singular values of $\bX$. Then it is equivalent to prove $\lambda_{\min}(\bM_1^\top\bM_1)$=$\lambda_{\min}(\bM_2^\top\bM_2)$, which is trivial since $z^2 = \bc^\top\bc$.
\end{proof}

We notice the Step ($A$) of Algorithm~\ref{alg:greedy-I}  finds the smallest singular value of a set of $n\times (l+1)$ matrices. By the lemma above, the problem amounts to determining the smallest singular values of upper triangular matrices of shape $(l+1)\times (l+1)$.


The first approximation of Algorithm~\ref{alg:greedy-I} is to approximate the smallest singular value of a matrix by the reciprocal of the largest two-norm of the rows of its inverse.
\begin{lemma}[Bound of Smallest Singular Value]
Given a nonsingular matrix $\bA\in\real^{n\times n}$ with the column partition of its inverse:
$$
\bA^{-1}=
\begin{bmatrix}
\ba_1^\top \\
\ba_2^\top \\
\vdots \\
\ba_n^\top 
\end{bmatrix}.
$$
Then it follows that
$$
\sigma_{\min}(\bA) \leq 
\mathop{\min}_{1\leq i\leq n } \frac{1}{\norm{\ba_i}}
\leq 
\sigma_{\min}(\bA) \sqrt{n}.
$$
\end{lemma}
The above lemma shows that the smallest singular value of a nonsingular matrix of order $n$ can be estimated up to a factor of $\sqrt{n}$. 

\begin{algorithm}[H] 
\caption{Greedy-I.1, Approximate Smallest Singular Value of Order $\sqrt{n}$ \citep{stewart1990incremental}} 
\label{alg:greedy-I_1} 
\begin{algorithmic}[1] 
\Statex Replace Step ($A$) of Algorithm~\ref{alg:greedy-I} as follows:
\State   ($A$). Find the next column $l+j$ from $\bR^{(l)}$ such that 
$$
\mathop{\min}_{h}
\norm{\be_h^\top 
\begin{bmatrix}
\bX & \by_j \\ 
\bzero & z_j
\end{bmatrix}^{-1}
}^{-1}
=
\mathop{\max}_{1\leq i \leq n-l}
\mathop{\min}_{h}
\norm{\be_h^\top 
\begin{bmatrix}
\bX & \by_i \\ 
\bzero & z_i
\end{bmatrix}^{-1}
}^{-1},
$$
where $z_i = \norm{\bz_i}$ and $\be_h$ is the $h$-th unit basis of $\real^{n}$.
\end{algorithmic} 
\end{algorithm}

Suppose the Greedy-I and Greedy-I.1 algorithms have the same submatrix $\bX$ in iteration $l$,
then the $\sigma_{\min}$ from Greedy-I is no smaller than the $\sigma_{\min}$ from Greedy-I.1. 
However, this is no guarantee that the $\sigma_{\min}$ of Greedy-I for next iteration will be  larger or equal to that of Greedy-I.1.
This is because the greedy algorithms are not globally optimal and they find the locally optimal solutions.

We need to calculate the inverse of an $(l+1)\times (l+1)$ matrix at step $(A)$ of Greedy-I.1 algorithm. To further reduce complexity, we notice that 
\begin{equation}\label{equation:greedy_i1_simp1}
\text{(Approximation 1)}
\gap
\begin{bmatrix}
	\bX & \by_i \\ 
	\bzero & z_i
\end{bmatrix}^{-1}
= 
\begin{bmatrix}
	\bX^{-1} & -\bX^{-1}\by_i z_i^{-1}  \\ 
	\bzero & z_i^{-1}
\end{bmatrix},
\end{equation}
where the upper left $l\times l$ block $\bX^{-1}$ has already been calculated from the previous iteration. 
Therefore, only the last column of the inverse needs to be computed for each $i\in\{1,2,\ldots, n-l\}$.

To further reduce the complexity, suppose $\sigma_{\min}$ is not small in iteration $l-1$, i.e., no row of $\bX$ in iteration $l$ can have a large norm.
Suppose further $\sigma_{\min}$ is also not small in iteration $l$, then for some $i\in\{1,2,\ldots, n-l\}$, we can find some component of the last column of Equation~\eqref{equation:greedy_i1_simp1} must be large in magnitude. This yields the second approximation
\begin{equation}\label{equation:greedy_i1_simp2}
\text{(Approximation 2)}
\gap
\norm{\be_h^\top 
\begin{bmatrix}
\bX & \by_j \\ 
\bzero & z_j
\end{bmatrix}^{-1}
}
\approx
\abs{
\left(\begin{bmatrix}
	-\bX^{-1}\by_i z_i^{-1} \\ 
	z_i^{-1}
\end{bmatrix}\right)_h
},
\end{equation}
where $(\bv)_h$ is the $h$-th element of the vector $\bv$. This yields the Greedy-I.2 algorithm.

\begin{algorithm}[H] 
\caption{Greedy-I.2, Approximate Greedy-I.1 \citep{stewart1990incremental}} 
\label{alg:greedy-I_2} 
\begin{algorithmic}[1] 
\Statex Replace Step ($A$) of Algorithm~\ref{alg:greedy-I} as follows:
\State   ($A$). Find the next column $l+j$ from $\bR^{(l)}$ such that 
$$
\mathop{\min}_{h}
\abs{
	\left(\begin{bmatrix}
		-\bX^{-1}\by_j z_j^{-1} \\ 
		z_j^{-1}
	\end{bmatrix}\right)_h
}^{-1}
=
\mathop{\max}_{1\leq i \leq n-l}
\mathop{\min}_{h}
\abs{
	\left(\begin{bmatrix}
		-\bX^{-1}\by_i z_i^{-1} \\ 
		z_i^{-1}
	\end{bmatrix}\right)_h
}^{-1},
$$
where $z_i = \norm{\bz_i}$.
\end{algorithmic} 
\end{algorithm}







==> end.tex <==
\backmatter
\clearpage

\pagestyle{empty}
\begin{center}
	\bfseries
\vspace{1cm}
	\Huge
	{\huge
		{Publisher: Eliva Press Global Ltd}}
	
{\huge
	{Email: info@elivapress.com}}
	
\vspace{1cm}
	\normalsize
	

\vspace{1cm}
%	\small BY\\
	
\vspace{1cm}
\vspace{1cm}
	\normalsize
	
\vspace{1cm}
	\large
All rights reserved
\end{center}



\clearpage
\pagestyle{empty}
\begin{flushleft}
	\large
\textbf{Eliva Press} is an independent international publishing house established for the publication and dissemination of academic works all over the world. Company provides high quality and professional serves for all of our authors.


\vspace{1cm}

Our Services:
Free of charge, open-minded, eco-friendly, innovational.

\vspace{1cm}

- Free standard publishing services (manuscript review, step-by-step book preparation, publication, distribution, and marketing).

- No financial risk. The author is not obliged to pay any hidden fees for publication.

- Editors. Dedicated editors will assist step by step through the projects. 

- Money paid to the author for every book sold. Up to 50\% royalties guaranteed. 

- ISBN (International Standard Book Number). We assign a unique ISBN to every Eliva Press book.

- Digital archive storage. Books will be available online for a long time. We don't need to have a stock of out titles. No unsold copies. Eliva Press uses environment friendly print on demand technology that limits the needs of publishing business. We care about environment and share these principles with our customers. 

- Cover design. Cover art is designed by a professional designer. 

- Worldwide distribution. We continue expanding our distribution channels to make sure that all readers have access to our books.



\bfseries
\vspace{1cm}
%\Huge
%{\nbtitlestretch\Huge
%\mytitle}

\vspace{1cm}
\normalsize

\vspace{4cm}

\vspace{1cm}

\normalsize


\huge
\bfseries
\gap\gap\qquad www.elivapress.com
\vspace{1cm}
\end{flushleft}



==> img-matricization.tex <==



























\begin{figure}[h]
	\centering
	\vspace{-0.35cm}
	\subfigtopskip=2pt
	\subfigbottomskip=2pt
	\subfigcapskip=-5pt
	\subfigure[Horizontal slices $\eX_{i,:,:}$]{\label{fig:third-matrix1}%
		\centering
		\begin{minipage}[b]{0.9\linewidth}
			\centering  
\begin{tikzpicture}
\pgfmathsetmacro{\cubex}{3}
\pgfmathsetmacro{\cubey}{2}
\pgfmathsetmacro{\cubez}{4}

%\draw[dotted,black,fill=white,fill opacity=0] (0,0,0) -- ++(-\cubex,0,0) -- ++(0,-\cubey,0) -- ++(\cubex,0,0) -- cycle;
\draw[dotted,black,fill=white,fill opacity=0] (0,0,0) -- ++(0,0,-\cubez/4*3) -- ++(0,-\cubey,0) -- ++(0,0,\cubez/4*3);
\draw[dotted,black,fill=white,fill opacity=0] (0,0,0) -- ++(-\cubex,0,0) -- ++(0,0,-\cubez/4*3) -- ++(\cubex,0,0);

%\draw[dotted,black,fill=white,fill opacity=0] (0,0,0) -- ++(-\cubex,0,0) -- ++(0,-\cubey,0) -- ++(\cubex,0,0) -- cycle;
\draw[dotted,black,fill=white,fill opacity=0] (0,0,0) -- ++(0,0,-\cubez/4*2) -- ++(0,-\cubey,0) -- ++(0,0,\cubez/4*2);
\draw[dotted,black,fill=white,fill opacity=0] (0,0,0) -- ++(-\cubex,0,0) -- ++(0,0,-\cubez/4*2) -- ++(\cubex,0,0);

%\draw[dotted,black,fill=white,fill opacity=0] (0,0,0) -- ++(-\cubex,0,0) -- ++(0,-\cubey,0) -- ++(\cubex,0,0) -- cycle;
\draw[dotted,black,fill=white,fill opacity=0] (0,0,0) -- ++(0,0,-\cubez/4) -- ++(0,-\cubey,0) -- ++(0,0,\cubez/4);
\draw[dotted,black,fill=white,fill opacity=0] (0,0,0) -- ++(-\cubex,0,0) -- ++(0,0,-\cubez/4) -- ++(\cubex,0,0);


\draw[black,fill=white,fill opacity=0] (0,0,0) -- ++(-\cubex,0,0) -- ++(0,-\cubey,0) -- ++(\cubex,0,0) -- cycle;
\draw[black,fill=white,fill opacity=0] (0,0,0) -- ++(0,0,-\cubez) -- ++(0,-\cubey,0) -- ++(0,0,\cubez) -- cycle;
\draw[black,fill=white,fill opacity=0] (0,0,0) -- ++(-\cubex,0,0) -- ++(0,0,-\cubez) -- ++(\cubex,0,0) -- cycle;

\draw (-\cubex/2,-\cubey*1.25,0) node {\scriptsize{\color{gray}$J$}};
\draw (-\cubex/2,-\cubey-0.2,0) node[rotate = 0] {{\color{gray!65}$\underbrace{\hspace{3cm}}$}};
\draw (-\cubex/2-1.2,-0.25,\cubez/2) node[rotate = 90] {\scriptsize{\color{gray}$I$}};
\draw (-\cubex/2-0.9,-0.25,\cubez/2) node[rotate = 270] {{\color{gray!65}$\underbrace{\hspace{2cm}}$}};
\draw (\cubex/2+0.3,-\cubey/2,1.7) node[rotate = 45] {\scriptsize{\color{gray}$K$}};
\draw (\cubex/2-0.2,-\cubey/2,1.1) node[rotate = 45] {{\color{gray!65}$\underbrace{\hspace{2.3cm}}$}};


\draw [-{Implies},double](\cubex,-\cubey/2) -- ++(1,0);
\pgfmathsetmacro{\cubexx}{6}
\draw[dotted,black,fill=white,fill opacity=0] (10,0,0) -- ++(-\cubex*3/4*3,0,0) -- ++(0,-\cubey,0) -- ++(\cubex*3/4*3,0,0) -- cycle;
\draw[dotted,black,fill=white,fill opacity=0] (10,0,0) -- ++(-\cubex*3/4*2,0,0) -- ++(0,-\cubey,0) -- ++(\cubex*3/4*2,0,0) -- cycle;
\draw[dotted,black,fill=white,fill opacity=0] (10,0,0) -- ++(-\cubex*3/4,0,0) -- ++(0,-\cubey,0) -- ++(\cubex*3/4,0,0) -- cycle;
\draw[black,fill=white,fill opacity=0] (10,0,0) -- ++(-\cubex*3,0,0) -- ++(0,-\cubey,0) -- ++(\cubex*3,0,0) -- cycle;
\end{tikzpicture}
		\end{minipage}%
	}
	\subfigure[Lateral slices $\eX_{:,j,:}$]{\label{fig:third-matrix2}%
		\centering
		\begin{minipage}[b]{0.8\linewidth}
			\centering 
\begin{tikzpicture}
\pgfmathsetmacro{\cubex}{3}
\pgfmathsetmacro{\cubey}{2}
\pgfmathsetmacro{\cubez}{4}

\draw[dotted,black,fill=white,fill opacity=0] (0,0,0) -- ++(0,0,-\cubez/4*3) -- ++(0,-\cubey,0) -- ++(0,0,\cubez/4*3);
\draw[dotted,black,fill=white,fill opacity=0] (0,0,0) -- ++(-\cubex,0,0) -- ++(0,0,-\cubez/4*3) -- ++(\cubex,0,0);

\draw[dotted,black,fill=white,fill opacity=0] (0,0,0) -- ++(0,0,-\cubez/4*2) -- ++(0,-\cubey,0) -- ++(0,0,\cubez/4*2);
\draw[dotted,black,fill=white,fill opacity=0] (0,0,0) -- ++(-\cubex,0,0) -- ++(0,0,-\cubez/4*2) -- ++(\cubex,0,0);

\draw[dotted,black,fill=white,fill opacity=0] (0,0,0) -- ++(0,0,-\cubez/4) -- ++(0,-\cubey,0) -- ++(0,0,\cubez/4);
\draw[dotted,black,fill=white,fill opacity=0] (0,0,0) -- ++(-\cubex,0,0) -- ++(0,0,-\cubez/4) -- ++(\cubex,0,0);


\draw[black,fill=white,fill opacity=0] (0,0,0) -- ++(-\cubex,0,0) -- ++(0,-\cubey,0) -- ++(\cubex,0,0) -- cycle;
\draw[black,fill=white,fill opacity=0] (0,0,0) -- ++(0,0,-\cubez) -- ++(0,-\cubey,0) -- ++(0,0,\cubez) -- cycle;
\draw[black,fill=white,fill opacity=0] (0,0,0) -- ++(-\cubex,0,0) -- ++(0,0,-\cubez) -- ++(\cubex,0,0) -- cycle;

\draw (-\cubex/2,-\cubey*1.25,0) node {\scriptsize{\color{gray}$J$}};
\draw (-\cubex/2,-\cubey-0.2,0) node[rotate = 0] {{\color{gray!65}$\underbrace{\hspace{3cm}}$}};
\draw (-\cubex/2-1.2,-0.25,\cubez/2) node[rotate = 90] {\scriptsize{\color{gray}$I$}};
\draw (-\cubex/2-0.9,-0.25,\cubez/2) node[rotate = 270] {{\color{gray!65}$\underbrace{\hspace{2cm}}$}};
\draw (\cubex/2+0.3,-\cubey/2,1.7) node[rotate = 45] {\scriptsize{\color{gray}$K$}};
\draw (\cubex/2-0.2,-\cubey/2,1.1) node[rotate = 45] {{\color{gray!65}$\underbrace{\hspace{2.3cm}}$}};


\draw [-{Implies},double](\cubex,-\cubey/2) -- ++(1,0);
\pgfmathsetmacro{\cubexx}{6}
\draw[dotted,black,fill=white,fill opacity=0] (\cubey*4,0,0) -- ++(-\cubey*3/4*3,0,0) -- ++(0,-\cubex,0) -- ++(\cubey*3/4*3,0,0) -- cycle;
\draw[dotted,black,fill=white,fill opacity=0] (\cubey*4,0,0) -- ++(-\cubey*3/4*2,0,0) -- ++(0,-\cubex,0) -- ++(\cubey*3/4*2,0,0) -- cycle;
\draw[dotted,black,fill=white,fill opacity=0] (\cubey*4,0,0) -- ++(-\cubey*3/4,0,0) -- ++(0,-\cubex,0) -- ++(\cubey*3/4,0,0) -- cycle;
\draw[black,fill=white,fill opacity=0] (\cubey*4,0,0) -- ++(-\cubey*3,0,0) -- ++(0,-\cubex,0) -- ++(\cubey*3,0,0) -- cycle;
\end{tikzpicture}
			
		\end{minipage}%
	}
	\subfigure[Frontal slices $\eX_{:,:,k}$]{\label{fig:third-matrix13}%
		\centering
		\begin{minipage}[b]{0.8\linewidth}
			\centering
\begin{tikzpicture}
\pgfmathsetmacro{\cubex}{3}
\pgfmathsetmacro{\cubey}{2}
\pgfmathsetmacro{\cubez}{4}


\draw[dotted,black,fill=white,fill opacity=0] (-\cubex/3*2,-\cubey,0) -- ++(0,\cubey,0) -- ++(0,0,-\cubez);
\draw[dotted,black,fill=white,fill opacity=0] (-\cubex/3,-\cubey,0) -- ++(0,\cubey,0) -- ++(0,0,-\cubez);

\draw[black,fill=white,fill opacity=0] (0,0,0) -- ++(-\cubex,0,0) -- ++(0,-\cubey,0) -- ++(\cubex,0,0) -- cycle;
\draw[black,fill=white,fill opacity=0] (0,0,0) -- ++(0,0,-\cubez) -- ++(0,-\cubey,0) -- ++(0,0,\cubez) -- cycle;
\draw[black,fill=white,fill opacity=0] (0,0,0) -- ++(-\cubex,0,0) -- ++(0,0,-\cubez) -- ++(\cubex,0,0) -- cycle;

\draw (-\cubex/2,-\cubey*1.25,0) node {\scriptsize{\color{gray}$J$}};
\draw (-\cubex/2,-\cubey-0.2,0) node[rotate = 0] {{\color{gray!65}$\underbrace{\hspace{3cm}}$}};
\draw (-\cubex/2-1.2,-0.25,\cubez/2) node[rotate = 90] {\scriptsize{\color{gray}$I$}};
\draw (-\cubex/2-0.9,-0.25,\cubez/2) node[rotate = 270] {{\color{gray!65}$\underbrace{\hspace{2cm}}$}};
\draw (\cubex/2+0.3,-\cubey/2,1.7) node[rotate = 45] {\scriptsize{\color{gray}$K$}};
\draw (\cubex/2-0.2,-\cubey/2,1.1) node[rotate = 45] {{\color{gray!65}$\underbrace{\hspace{2.3cm}}$}};


\draw [-{Implies},double](\cubex,-\cubey/2) -- ++(1,0);
\pgfmathsetmacro{\cubexx}{6}
\draw[dotted,black,fill=white,fill opacity=0] (\cubez*4,0,0) -- ++(-\cubez*3/4*3,0,0) -- ++(0,-\cubex,0) -- ++(\cubez*3/4*3,0,0) -- cycle;
\draw[dotted,black,fill=white,fill opacity=0] (\cubez*4,0,0) -- ++(-\cubez*3/4*2,0,0) -- ++(0,-\cubex,0) -- ++(\cubez*3/4*2,0,0) -- cycle;
\draw[dotted,black,fill=white,fill opacity=0] (\cubez*4,0,0) -- ++(-\cubez*3/4,0,0) -- ++(0,-\cubex,0) -- ++(\cubez*3/4,0,0) -- cycle;
\draw[black,fill=white,fill opacity=0] (\cubez*4,0,0) -- ++(-\cubez*3,0,0) -- ++(0,-\cubex,0) -- ++(\cubez*3,0,0) -- cycle;
\end{tikzpicture}
		\end{minipage}%
	}
	\caption{Slices of a third-order tensor $\eX\in \real^{I\times J\times K}$. The \textbf{darker}, the larger the index.}
	\label{fig:thifd-matrix123}
\end{figure}

%\begin{figure}[htbp]
%\centering
%\resizebox{0.4\textwidth}{!}{%
%
%}
%\caption{Index of the CP decomposition of a third-order tensor: $\eX\approx\llbracket \bA,\bB,\bC\rrbracket$.}
%\label{fig:cpnceo-matricization}
%\end{figure}

